Many Electrons and the Photon Field -- The many-body structure of nonrelativistic quantum electrodynamics

Recent experimental progress in the field of cavity quantum electrodynamics allows to study the regime of strong interaction between quantized light and complex matter systems. Due to the coherent coupling between photons and matter-degrees of freedom, polaritons -- hybrid light-matter quasiparticles -- emerge, which can significantly influence matter properties and complex processes such as chemical reactions (strong coupling). In this thesis we propose a way to overcome these problems by reformulating the coupled electron-photon problem in an exact way in a different, purpose-build Hilbert space, where no longer electrons and photons are the basic physical entities but the polaritons. Representing an N-electron-M-mode system by an N-polariton wave function with hybrid Fermi-Bose statistics, we show explicitly how to turn electronic-structure methods into polaritonic-structure methods that are accurate from the weak to the strong-coupling regime. We elucidate this paradigmatic shift by a comprehensive review of light-matter coupling, as well as by highlighting the connection between different electronic-structure methods and quantum-optical models. This extensive discussion accentuates that the polariton description is not only a mathematical trick, but it is grounded in a simple and intuitive physical argument: when the excitations of a system are hybrid entities a formulation of the theory in terms of these new entities is natural. Finally, we discuss in great detail how to adopt standard algorithms of electronic-structure methods to adhere to the new hybrid Fermi-Bose statistics. Guaranteeing the corresponding nonlinear inequality constraints in practice requires a careful development, implementation and validation of numerical algorithms. This extra numerical complexity is the price we pay for making the coupled matter-photon problem feasible for first-principle methods.

==> intro_physical_setting.tex <==
% [Polaritons and QED]
% Polaritons and Quantum-Electrodynamics from First Principles

%\newpage
%As outlined in the introduction, our research aims for a general understanding of coupled light-matter systems from first principles, which is a broad topic that has not been studied much in the past. To approach this problem, we focus our discussion mostly on a simplified physical setting, which we motivate, introduce and discuss from a first-principles perspective in this part.

%Specifically, we aim to describe the \emph{equilibrium} properties of molecular \emph{many-electron systems} that are coupled via their \emph{dipole} to a \emph{few modes} of the electromagnetic field. This means that we include in principle the whole (equilibrium) \emph{electronic-structure} of the matter systems, which is sufficient to understand, e.g., the equilibrium structure of molecules and materials and even chemical processes such as certain chemical reactions. With regard to the description of light and the light-matter interaction, this setting is more exclusive. The dipole-approximation leads, e.g., to a spatially constant light-matter interaction. And only special experimental setups such as \emph{optical cavities} create scenarios that are well described taking only a few electromagnetic modes into account. We therefore call this physical setting \emph{cavity QED}.


%\vspace{0.5cm}
%This part consists of three chapters. In Ch. ~\ref{sec:intro} we motivate the research on first-principles approaches for cavity QED by recent experimental results that are not satisfactorily understood by the standard theoretical approaches (Sec.~\ref{sec:intro:experiment_strong_coupling}). We discuss these standard approaches and their limitations in a bit more detail in  Sec.~\ref{sec:intro:cavity_qed_models}. In the last section (Sec.~\ref{sec:intro:light_matter}), we broaden the perspective and outline the basics of Pauli-Fierz theory with the goal to define a theoretical framework that is suitable for the first-principles perspective. 
%
%Having introduced the standard approaches to describe the phenomena of cavity QED, we then dedicate one chapter (Ch. ~\ref{sec:est}) to the introduction of the first-principles perspective on physical systems. We do this with the example of the many-electron problem, for which most of the known first-principles methods have been developed. Such electronic-structure methods be the most important source for our first-principles description of the coupled light-matter problems and we discuss this topic in an appropriate depth.
%We introduce in Sec.~\ref{sec:est:general} the electronic-structure Hamiltonian, the many-electron wave function and its expansion in terms of Slater determinants that accounts for the antisymmetry of electrons. We show how we can utilize these tools to determine in principle the ground state of any many-electron system by a variational minimization. We then illustrate that such a minimization is infeasible in practice (many-body problem), which is the principal motivation for the research on (approximate) first-principles methods.
%We then present three different approaches to describe many-electron systems: Hartree-Fock theory (Sec.~\ref{sec:est:hf}), density-functional theory (Sec.~\ref{sec:est:dft}) and reduced density matrix functional theory (Sec.~\ref{sec:est:rdms:rdmft}) that is based on the concept of reduced density matrices (Sec.~\ref{sec:est:rdms:general}). We derive the corresponding energy functionals and equations that determine the ground state. For all approaches, we discuss the strengths and limitations. We also remark on practical issues with regard to numerical solutions. We conclude the section with a concrete example to compare all the introduced approaches (Sec.~\ref{sec:est:comparison}).
%
%In the last chapter (Ch.~\ref{sec:qed_est}), we discuss the first-principles perspective on coupled light-matter systems in the cavity QED setting. The principal strategy for that be to generalize the introduced concepts and methods of electronic-structure theory to the coupled electron-photon space. We start in Sec.~\ref{sec:qed_est:general} with the proper introduction of the minimization problem of the cavity QED Hamiltonian, including the symmetries of the corresponding wave function. We then illustrate the approximate wave function description with the example of mean field theory, i.e., the generalization of Hartree-Fock theory. In Sec.~\ref{sec:qed_est:qedft}, we then discuss the generalization of density functional theory to coupled light matter problems and finally in Sec.~\ref{sec:qed_est:rdms}, we introduce the reduced density matrix description. For all approaches, we highlight the new challenges that arise from the simultaneous description of two particle species.
